A Method for Curation of Web-Scraped Face Image Datasets

Web-scraped, in-the-wild datasets have become the norm in face recognition research. The numbers of subjects and images acquired in web-scraped datasets are usually very large, with number of images on the millions scale. A variety of issues occur when collecting a dataset in-the-wild, including images with the wrong identity label, duplicate images, duplicate subjects and variation in quality. With the number of images being in the millions, a manual cleaning procedure is not feasible. But fully automated methods used to date result in a less-than-ideal level of clean dataset. We propose a semi-automated method, where the goal is to have a clean dataset for testing face recognition methods, with similar quality across men and women, to support comparison of accuracy across gender. Our approach removes near-duplicate images, merges duplicate subjects, corrects mislabeled images, and removes images outside a defined range of pose and quality. We conduct the curation on the Asian Face Dataset (AFD) and VGGFace2 test dataset. The experiments show that a state-of-the-art method achieves a much higher accuracy on the datasets after they are curated. Finally, we release our cleaned versions of both datasets to the research community.

==> figures/mislabeled.tex <==
\begin{figure}[ht!]
    \centering
    \begin{subfigure}[b]{.49\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/ml.jpg}
        \caption{Correct image: malong}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.49\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/zjk.jpg}
        \caption{Wrong image: zhangjike}
    \end{subfigure}
    \caption{Mislabelled image, later deleted in the mislabelled cleaning stage.}
\end{figure}

==> figures/mislabeled_examples.tex <==
\begin{figure*}[ht!]
    \begin{subfigure}[b]{.45\textwidth}
        \centering
        \centering
        \begin{subfigure}[b]{.49\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{images/anhu_0038.jpg}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{.49\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{images/anhu_0039.jpg}
        \end{subfigure}
        \caption{Correct images}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.45\textwidth}
        \centering
        \centering
        \begin{subfigure}[b]{.49\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{images/anhu_0158.jpg}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{.49\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{images/anhu_0048.jpg}
        \end{subfigure}
        \caption{Mislabelled images}
    \end{subfigure}
    \caption{Images in the subject folder ``anhu''.}
\end{figure*}

==> figures/near_duplicate_example.tex <==
\begin{figure}[t]
    \begin{subfigure}[b]{\columnwidth}
        \centering
        \centering
        \begin{subfigure}[b]{.24\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{images/adu_near_duplicate/adu_0022.jpg}
            \caption{100\%}
        \end{subfigure}
        \begin{subfigure}[b]{.24\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{images/adu_near_duplicate/adu_0035.jpg}
            \caption{32.84\%}
        \end{subfigure}
        \begin{subfigure}[b]{.24\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{images/adu_near_duplicate/adu_0084.jpg}
            \caption{41.87\%}
        \end{subfigure}
        \begin{subfigure}[b]{.24\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{images/adu_near_duplicate/adu_0085.jpg}
            \caption{18.66\%}
        \end{subfigure}
        \vspace{1em}
    \end{subfigure}
    \vfill
    \begin{subfigure}[b]{\columnwidth}
        \vspace{-2em}
        \centering
        \begin{subfigure}[b]{.24\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{images/adu_near_duplicate/adu_0095.jpg}
            \caption{35.06\%}
        \end{subfigure}
        \begin{subfigure}[b]{.24\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{images/adu_near_duplicate/adu_0096.jpg}
            \caption{40.61\%}
        \end{subfigure}
        \begin{subfigure}[b]{.24\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{images/adu_near_duplicate/adu_0097.jpg}
            \caption{30.71\%}
        \end{subfigure}
        \begin{subfigure}[b]{.24\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{images/adu_near_duplicate/adu_0098.jpg}
            \caption{28.79\%}
        \end{subfigure}
        \vspace{1em}
    \end{subfigure}
    \vfill
    \begin{subfigure}[b]{\columnwidth}
        \vspace{-2em}
        \centering
        \begin{subfigure}[b]{.24\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{images/adu_near_duplicate/adu_0138.jpg}
            \caption{24.12\%}
        \end{subfigure}
        \begin{subfigure}[b]{.24\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{images/adu_near_duplicate/adu_0180.jpg}
            \caption{9.34\%}
        \end{subfigure}
        \begin{subfigure}[b]{.24\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{images/adu_near_duplicate/adu_0195.jpg}
            \caption{12.72\%}
        \end{subfigure}
        \begin{subfigure}[b]{.24\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{images/adu_near_duplicate/adu_0205.jpg}
            \caption{33.07\%}
        \end{subfigure}
    \end{subfigure}
    \vspace{-1em}
    \caption{Example of near-duplicate images of subject ``adu''. These images may seem identical, but they are not. The caption below each image represent the percentage of same pixels between each image and image (a).}
    \vspace{-1em}
    \label{fig:near_duplicates}
\end{figure}

==> figures/quality_images.tex <==
\begin{figure}[ht!]
    \centering
    \begin{subfigure}[b]{.49\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/1.jpg}
        \caption{Bad pose angle}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.49\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/lr.jpg}
        \caption{Blurry image}
    \end{subfigure}
    \caption{Images later deleted in the mislabelled cleaning stage.}
\end{figure}

==> figures/wrong_subject.tex <==
\begin{figure}[ht!]
    \centering
    \begin{subfigure}[b]{.47\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/zhb.jpg}
        \caption{Image in the folder of "shenxue}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.49\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/sx.png}
        \caption{Image of "shenxue" and "zhaohongbo" from the Internet}
    \end{subfigure}
    \caption{Wrong subject folder}
\end{figure}
